ClarifyGPT: Empowering LLM-based Code Generation with Intention Clarification

We introduce a novel framework named ClarifyGPT, which aims to enhance code generation by empowering LLMs with the ability to identify ambiguous requirements and ask targeted clarifying questions. In particular, ClarifyGPT first detects whether a given requirement is ambiguous by performing a code consistency check. If it is ambiguous, ClarifyGPT prompts an LLM to generate targeted clarifying questions. After receiving question responses, ClarifyGPT refines the ambiguous requirement and inputs it into the same LLM to generate a final code solution. To evaluate our ClarifyGPT, we first conduct a human evaluation involving ten participants who use ClarifyGPT for code generation on two publicly available benchmarks: MBPP-sanitized and MBPP-ET. The results show that ClarifyGPT elevates the performance (Pass@1) of GPT-4 from 70.96% to 80.80% on MBPP-sanitized. Furthermore, to perform large-scale automated evaluations of ClarifyGPT across different LLMs and benchmarks without requiring user participation, we introduce a high-fidelity simulation method to simulate user responses. The automated evaluation results also demonstrate that ClarifyGPT can significantly enhance code generation performance compared to the baselines. In particular, ClarifyGPT improves the average performance of GPT-4 and ChatGPT across four benchmarks from 68.02% to 75.75% and from 58.55% to 67.22%, respectively. We believe that ClarifyGPT can effectively facilitate the practical application of LLMs in real-world development environments.

==> sec/intro.tex <==
\section{Introduction}
Code generation aims to produce a code snippet that satisfies the user's intent expressed in a natural language requirement. This task, which offers potential cost savings, accelerates programming activities, and facilitates software development, has consequently garnered attention across various domains, e.g., natural language processing, artificial intelligence, and software engineering. Recent efforts tackle this task by leveraging Large Language Models (LLMs) with billions of parameters, such as ChatGPT\cite{} and CodeGen\cite{}. The LLMs take the natural language requirements (i.e., prompts) as inputs and output the corresponding code snippets, achieving remarkable progress in code generation. 

However, in real-world \lin{practice} scenarios, \lin{due to the diversity of user experience and perspective, it is inevitable that the requirements written by users might be ambiguous or insufficient.}
{For example}, %\song{can you move the example here? or you can use a different simplified example only for the motivation} 
the requirement \textit{"Write a function to sort a list of elements"} does not specify whether the user intends for the list to be sorted in ascending or descending order. 
Current LLMs do not handle such ambiguous requirements: they rarely ask users to clarify these requirements and instead directly generate programs that may deviate from the users’ needs~\cite{kuhn2023clam}.
\lin{Current LLMs-based code generation approaches lack the mechanism of clarifying unclear requirements \lin{cite 2-3 papers}, i.e., they directly generate programs according to those unclear requirements regardless of interactive clarification.}
% They usually infer what users intended and produce code snippets that may not be consistent with the actual user's intentions\cite{}. So we can see ChatGPT \cite{} directly writes a function that sorts the list in descending order, which fails to pass the provided test cases.
In contrast, when human developers encounter ambiguous requirements, they typically seek additional information by interactively asking clarifying questions to the users. For the above example, a simple clarifying question such as \textit{"Should the sorting be in ascending or descending order?"} could help disambiguate the requirement. %the developer can get clear feedback from the user and write a correct code solution.

In light of this observation, we argue that empowering LLMs with the ability to automatically ask clarifying questions for ambiguous requirements is necessary for improving the quality and efficiency of code generation. However, it is quite challenging to empower LLMs with this ability due to the following barriers.
% Although important, there are few studies dedicated to it. GPT-Engineer\footnote{https://github.com/AntonOsika/gpt-engineer}, the most related work, is a recent open-source Github repository. It utilizes manual-designed instructions to elicit LLMs to ask clarifying questions for the input user requirements, and then generates code snippets based on user feedback. While existing studies achieve success more or less, two challenges remain unresolved: 
\textbf{(1) When to Ask Clarifying Questions?} In practical development environments, numerous requirements exist, including both ambiguous and unambiguous ones. Failure to concentrate on questioning only the ambiguous requirements can lead to unnecessary interactions between LLMs and users regarding well-defined requirements. These unnecessary interactions, in turn, can diminish efficiency and compromise the user experience.\lin{describe the GPT-engieer issue?}
% For example, 
\textbf{(2) What Clarifying Questions Should be Asked?} The quality of clarifying questions also influences the efficiency and performance of code generation. Precisely and targeted questions aid users in expressing their intents clearly, ensuring that the obtained responses are directly relevant to the ambiguities present in the requirements. Vague or broad questions increase the risk of obtaining off-topic or irrelevant responses, potentially hindering LLMs from comprehending user intents.
% For example,

To address these challenges, in this paper, we propose a novel framework called {\tool} that enhances LLM-based code generation via requirement clarification.
% enables LLMs to automatically detect ambiguous requirements and further generate targeted clarifying questions for them. 
\mfw{Specifically, regarding the first challenge, we are motivated by the observation that a clear requirement should leave no room for interpretation, ensuring that everyone involved in the project understands it in the same way; while an ambiguous requirement can lead to disagreements among developers. 
\lin{this statement is too strong}
\lin{Specifically, }
Therefore, we make the assumption that if a large number of code solutions with varying functionalities are generated by an LLM in response to a user requirement, the requirement needs further clarification. 
In light of this assumption, {\tool} conducts a two-step code consistency check to detect ambiguous requirements. 
In the first step, {\tool} aims to generate numerous high-quality test inputs for a given requirement. 
In the second step, {\tool} inputs the given requirement into an LLM to sample $n$ code solutions and checks whether they produce identical outputs when tested with the generated input. 
If the outputs are not identical, {\tool} determines that the requirement requires further clarification; and vice versa. 
For the second challenge, {\tool} initially directs LLMs to analyze the factors contributing to the ambiguity of the given requirement by comparing code solutions with different functionalities. Subsequently, it formulates targeted clarifying questions based on the results of this analysis. Our intuitive rationale is that, in software development, code solutions represent specific implementations of requirements. If a requirement is ambiguous, different developers may interpret it differently and consequently write different code. By comparing these different code implementations, potential points of ambiguity in the requirements can be readily identified.  After detecting the points of ambiguity in the requirements, the LLMs can generate targeted clarifying questions for them.} Finally, {\tool} refines the original requirement based on the generated questions and their responses and generates the final code solution. 


% After that {\tool} refines the ambiguous requirements with answers to their clarifying questions and generates code that could fulfill the users' intentions. {\tool} consists of two components: Ambiguous Requirements Identification and Clarification Generation. In the Ambiguous Requirements Identification component,
\song{see comments}
%这里说一下我们的assumption，就说我们认为 ambiguous 的 requirement 可以使大模型产生不同logic 的 代码 with different functionalities？ threats to validity 里面也要说一下
%还有一个问题，就是 如果LLM 对 ambiguous requirement 的 理解是 deterministic的，是不是产生的solutions 是一致的呢？这个是不是就得 解释一下 LLM是怎么 guess 或者 infer intent的了，不是一个 determinstic的过程，看看有没有citation    

% we first input a given requirement into an LLM and sample $n$ code solutions. By conducting functional consistency checks on the sampled codes, we determine whether the requirement is ambiguous. If the functionalities of these sampled codes are inconsistent, the requirement is seen as an ambiguous requirement, and vice versa.
% The motivation behind is that a clear requirement should leave no room for interpretation, ensuring that everyone involved in the project understands it in the same way; while an ambiguous requirement can lead to disagreements among developers. 
% In the Clarification Generation component, we feed the functionally inconsistent code generated in the previous step into the same LLM. Then, the LLM analyzes the reasons behind the inconsistent code functionality, identifies which expressions in the requirements are ambiguous, and formulates targeted clarifying questions to improve requirement clarity. Finally, {\tool} refines the original requirement based on the generated questions and their responses and generates the final code solution. 
% Besides, due to the involvement of human participants, evaluating {\tool} could be very expensive and hard to reproduce. To perform automated evaluations of {\tool} across different LLMs and benchmarks without requiring user participation, we introduce a high-fidelity simulation method to simulate user feedback. 

To assess the effectiveness of {\tool}, we first apply GPT-4~\cite{} to {\tool} and recruit ten participants to evaluate its performance on two public benchmarks (MBPP-sanitized\cite{}, and MBPP-ET\cite{}). The human evaluation results show that {\tool} achieves a relative improvement of up to 9.53\% in Pass@1 compared to the best-performing baseline. Besides, due to the involvement of human participants, evaluating {\tool} could be very expensive and hard to reproduce. To perform automated evaluations of {\tool} across different LLMs and benchmarks without requiring user participation, we introduce a high-fidelity simulation method to simulate user feedback. We then conduct comprehensive experiments on four benchmarks (HumanEval\cite{}, HumanEval-ET\cite{}, MBPP-sanitized, and MBPP-ET) using two state-of-the-art LLMs (i.e., GPT-4 and ChatGPT~\cite{}). The results demonstrate that, in comparison with the best-performing baseline, {\tool} achieves an average improvement of 8.41\% and 7.56\% across two LLMs for the four benchmarks, respectively.
% We apply {\tool} to two LLMs (i.e., GPT-4~\cite{} and ChatGPT~\cite{}) and evaluate their performance on four public benchmarks (HumanEval\cite{}, HumanEval-ET\cite{}, MBPP-sanitized\cite{}, and MBPP-ET\cite{}). Experimental results show that {\tool} achieves higher code generation performance than baselines across two LLMs and four benchmarks. Specifically, compared with the best-performing base-
% line, {\tool} achieves an average improvement of 8.95\%, 7.49\%, 6.95\%, and 8.56\% on four benchmarks, respectively. In human evaluation, compared to the best-performing baselines, {\tool} also achieves a relative improvement of up to 11.40\% in Pass@1 compared to the best-performing baseline.
Our main contributions are outlined as follows:   
\begin{itemize}%[leftmargin=*]
    \item \textbf{Framework}: We propose a novel framework, named {\tool}, which enables LLMs to detect ambiguous requirements and formulate targeted clarifying questions. {\tool} refines the ambiguous requirements based on the answers to clarifying questions and further generates code solutions.

    \item \textbf{User Simulation}: We introduce a user simulation method for producing high-fidelity simulated answers to the clarifying questions, which facilitates automated evaluations of {\tool} across different LLMs and benchmarks, eliminating the necessity for direct user participation.
    
    \item \textbf{Evaluation}: We conduct extensive experiments on four widely-used benchmarks to show that, {\tool} achieves substantial improvements across different models and benchmarks. A human evaluation further confirms the significant potential of applying {\tool} in real-world practice.
    
    \item \textbf{Data}: publicly accessible dataset and source code~\cite{website} to facilitate the replication of our study and its application in extensive contexts.
\end{itemize} 
 
% \lin{Give the paper structure introduction if have space} 

==> sec/motivation.tex <==
\section{Motivating Examples} 
\label{sec:moti}

To explain our motivations for designing {\tool}, we select two representative examples from two popular code generation benchmarks (i.e., HumanEval and MBPP), as shown in Figure \ref{fig:motivation}. Each input requirement consists of a function signature and a NL description. We take the ChatGPT\cite{} as the base model and utilize two baselines and {\tool} to generate a code solution for each input requirement.

For the first example taken from MBPP\cite{}, as we analyzed earlier, the description \textit{``write a function to sort a list of elements''} does not specify whether this function should be sorted in ascending or descending order. The default ChatGPT directly generates a code solution that sorts the given list in descending order, which fails to pass the ground-truth test cases. GPT-Engineer\footnote{https://github.com/AntonOsika/gpt-engineer} poses five clarifying questions and generates a correct code solution based on the user responses. However, some of those questions are uninformative and can be answered by the information in the given requirement. For instance, the answer to the third question \textit{``Are there any specific constraints for the sorting algorithm?''} can be inferred by the function name \textit{comb\_sort} mentioned in the function signature. The fifth question \textit{``Are there any preferred programming language?''} also seems trivial, since we can easily know that the function should be implemented in Python based on the syntax of the function signature. Answering these questions cannot obtain additional information; instead, it generates superfluous dialogues that are detrimental to the user experience. Furthermore, it results in an increase in token counts for both the LLMs' input and output, consequently escalating operational expenses. By contrast, {\tool} 








% In light of the observation, we consider that if we can diversely enrich the original prompts in the pre-direct, and select the optimal output in the post-optimize, the performance of code-LLMs is likely to improve.  
% Therefore, in this work, we propose {\tool}, an approach for improving the performance of code-LLMs via pre-direct and post-optimize, which 
% % leverages seven hand-crafted instructions
% {leverages a set of empirically pre-defined instructions} to augment the original prompts with diverse and valuable information and a similarity-based re-ranking method to recommend the optimal code.

% \begin{figure}[htbp]
% % \vspace{-0.2cm}
% \centering
% \includegraphics[width=\textwidth]{fig/motivation_example.png}
% % \vspace{-0.8cm}
% \caption{Motivating Examples of our {\tool}.}
% % need refine
% % \vspace{-0.6cm}
% \label{fig:motivation}
% \end{figure}

==> sec/todo.tex <==
Related work
implementation
approach figure
website

==> tab/mutate-input.tex <==
\begin{table}[t!]
\caption{List of basic type-aware mutations over input $x$ \cite{DBLP:journals/corr/abs-2305-01210}}
\label{tab:type-aware}
\begin{tabular}{l|l|l|l}
\hline
\multicolumn{1}{c|}{\textbf{Type}} & \multicolumn{1}{c|}{\textbf{Mutation}}& \multicolumn{1}{c|}{\textbf{Type}}         & \multicolumn{1}{c}{\textbf{Mutation}}        \\ \hline
\multirow{2}{*}{$int|float$}  & \multirow{2}{*}{Returns $x \pm 1$}   & \multicolumn{1}{c|}{\multirow{2}{*}{$List$}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}} $\left \{\begin{matrix} Remove/repeat \: a \: random \:  item \:  x[i] \\ Insert/replace \:  x[i]\: with \: Mutate(x[i])\\ \end{matrix} \right$ \end{tabular}}  \\
&   & \multicolumn{1}{c|}{}    &           \\ \hline
$bool$              & Returns a random $boolean$              & $Tuple$  & Returns $Tuple(Mutate(List(x)))$$                \\ \hline
$NoneType$          & Returns $None$        & $Set$    & Returns $Set(Mutate(List(x)))$\\ \hline
\multirow{3}{*}{$str}  & \multirow{3}{*}{\begin{tabular}[l]{@{}l@{}} $\left \{\begin{matrix}
Remove \: a \: substring \: s
\\Repeat \: a \: substring \: s
\\Replace \: s \: with \: Mutate(s) 
\end{matrix} \right$ 
\end{tabular}} 
& \multirow{3}{*}{Dict} & \multirow{3}{*}{\begin{tabular}[l]{@{}l@{}} 
$\left \{\begin{matrix}
Remove \: a \: key/value \: pair \: k \rightarrow v
\\Update \: k  \rightarrow v \: to \: k \rightarrow Mutate(v)
\\Insert \: Mutate(k) \rightarrow Mutate(v)\\ \end{matrix} \right$ \end{tabular}} \\
&   &        &           \\
&   &        &           \\ \hline
\end{tabular} 
\end{table}

==> tab/test.tex <==
\begin{table*}[htbp!]
\renewcommand\arraystretch{1.3}
\centering
\caption{The comparison results of variants and {\tool}.}
\label{table:RQ3}
\resizebox{\textwidth}{!}{
\begin{tabular}{ccccccc} 
\toprule
\multicolumn{2}{c}{Methods}                                      & HumanEval               & HumanEval-ET            & MBPP-sanitized          & MBPP-ET                 & Average                  \\ 
\hline
\multirow{5}{*}{ChatGPT} & Default                               & 64.63                   & 57.32                   & 65.57                   & 46.68                   & 58.55                    \\ \cline{2-7}
                         & {\tool} (zero-shot)  & 65.85                   & 58.13                   & 67.07                   & 48.01                   & 59.77                    \\
                         & {\tool} (one-shot)   & 72.80                   & 60.98                   & 70.96                   & 51.52                   & 64.07                    \\
                         & {\tool} (two-shot)   & 73.92         & 63.21                   & 72.60                   & 53.63                   & 65.84                    \\
                         & {\tool} (three-shot) & \textbf{\textbf{74.39}} & \textbf{\textbf{64.84}} & \textbf{\textbf{74.08}} & \textbf{\textbf{55.58}} & \textbf{\textbf{67.22}}  \\ 
\hline
\multirow{5}{*}{GPT-4}   & Default                               & 78.86                   & 70.73                   & 70.96                   & 51.52                   & 68.02                    \\ \cline{2-7}
                         & {\tool} (zero-shot)  & 79.26                   & 70.73                   & 72.13                   & 52.22                   & 68.59                    \\
                         & {\tool} (one-shot)   & 83.93                   & 72.76                   & 75.88                   & 55.97                   & 72.14                    \\ 
                         & {\tool} (two-shot)   & 85.15                   & 75.61                   & 77.75                   & 56.67                   & 73.80                    \\
                         & {\tool} (three-shot) & \textbf{\textbf{87.80}} & \textbf{\textbf{78.05}} & \textbf{\textbf{78.69}} & \textbf{\textbf{58.47}} & \textbf{\textbf{75.75}}  \\
\bottomrule
\end{tabular}
}
\end{table*}
\begin{table}
    \centering
    \begin{tabular}{cccccc}
         &  &  &  &  & \\
         &  &  &  &  & \\
         &  &  &  &  & \\
         &  &  &  &  & \\
         &  &  &  &  & \\
         &  &  &  &  & \\
         &  &  &  &  & \\
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

